The Experiment for Cryogenic Large-aperture Intensity Mapping (EXCLAIM)

The EXperiment for Cryogenic Large-Aperture Intensity Mapping (EXCLAIM) is a cryogenic balloon-borne instrument that will survey galaxy and star formation history over cosmological time scales. Rather than identifying individual objects, EXCLAIM will be a pathfinder to demonstrate an intensity mapping approach, which measures the cumulative redshifted line emission. EXCLAIM will operate at 420-540 GHz with a spectral resolution R=512 to measure the integrated CO and [CII] in redshift windows spanning 0 < z < 3.5. CO and [CII] line emissions are key tracers of the gas phases in the interstellar medium involved in star-formation processes. EXCLAIM will shed light on questions such as why the star formation rate declines at z < 2, despite continued clustering of the dark matter. The instrument will employ an array of six superconducting integrated grating-analog spectrometers (micro-spec) coupled to microwave kinetic inductance detectors (MKIDs). Here we present an overview of the EXCLAIM instrument design and status.

==> scrap.tex <==
% in an all-cryogenic telescope (\floattemp) to achieve near background-limited sensitivity

%The telescope is coupled to a receiver with 6 on-chip MKID spectrometers.%Flights from Palestine, TX provide good overlap with BOSS-North, while later flights from Ft. Sumner, NM provide access to BOSS-South and the Stripe 82 region.

%In addition to providing low photon background, the dewar holds the mirror and its mounts at a stable and uniform temperature. 
% EXCLAIM optics are additionally recessed in the dewar relative to ARCADE II.

%  by ConFlat and indium seals. We use a superfluid-tight high-current copper $3/4\”$ feedthrough with a ceramic-metal seal as thermal feedthrough for the \floattemp\ bath. 

%Off-axis $F/1.3$ Gregorian reflectors feed a single silicon lens through a stop. The lens slows the optics to the $F/2.8$ required for optimal coupling to the detectors. The stop tightly controls the illumination of the primary and limits stray light to well-defined black\citep{2008IJIMW..29...51W} baffles at \floattemp. The unobstructed design minimizes scattering. The optics tube accommodates a two-layer magnetic shield. The lens has a single-layer AR meta-material \citep{2013ApOpt..52.8747D}. 

% The lenslet has $4$\,mm diameter and has a $650\,\mu{\rm m}$ extension. 
% We will use a one-lens design to couple to the telescope. 

%Spectral calibration and stability are a premium for IM experiments \citep{2015ApJ...815...51S}. In addition to low background, the float environment provides stable loading, which supports stable channel responsivity. We will use a reverse bolometer \citep{2002SPIE.4486..209B} to provide periodic broadband calibration spectra to maintain inter-channel stability. The absolute response will be calibrated in the lab using a beam-filling cryogenic blackbody of loaded stycast cones. 

% An on-chip planar slot antenna (Fig.\,\ref{fig:r64photo}) with an extended hyper-hemispherical Si lens receives the light from the EXCLAIM telescope optics.

%Furthermore, the antenna-coupled approach used by \mspec\ (and other on-chip spectrometers) has advantages for cryogenic balloon or space MKID-based spectrometers, where high-sensitivity is needed. A direct-coupled MKID must meet multiple constraints on the inductor geometry, limiting optimization for low NEP.

% The electronics use custom MKID firmware on the second generation Reconfigurable Open Architecture Computing Hardware (ROACH-2) board developed by the CASPER collaboration and MUSIC digital-to-analog (DAC) and analog-to-digital (ADC) boards \nb{[CITE]}. 

%Each of the six spectrometers requires one readout module. 
%In parallel, we are investigating an RFSoC\footnote{\verb+https://www.xilinx.com/products/silicon-devices/soc/rfsoc.html+} readout for lower power and higher bandwidth.
%The total readout power requirement exceeds BLAST-TNG (5 modules) but smaller than EBEX \citep{2018ApJS..239....9T}. \citet{2016JAI.....541003G} describes thermal interfaces and dissipation. 

%, subject to requirements that 1) it spatially sample the beam in ${\rm FWHM}/3$ pixels, 2) the maximum rotation rate is $<2$\,deg/sec demonstrated in the PIPER gondola, 3) the $488$\,Hz readout samples the beam at the scan rate. Star camera solutions remain possible at the $2$\,deg/sec rotation rate.

% , and the Palestine, TX survey spans $8h-16h$\,RA centered on $57^\circ$\,Dec.

% A sensitivity forecast for an instrument with MKID detectors requires several considerations that are different from instruments with Transition-Edge Sensors (TESs), which typically specify a dark noise-equivalent power (NEP). This is because 
% the antenna-coupled MKID provides no access or electronic analogs (such as Joule power) to optical power absorbed by the MKIDs \nb{(is this quite true? not sure I follow what is meant here- EB)}
% \nb{(a TES could also have 1/f? do you mean loading dependent or dominated by 1/f? - EB)}
% We consider an NEP of the spectrometers under expected optical loading that is parameterized as a factor  

%The science case is self-contained without recent Extended-BOSS releases, but these will be included in survey planning. 

%Threshold science is achieved for a detection of CO in at least two redshift bins, and a definitive detection ($7\sigma$) at the level of [CII] suggested by \citet{2019arXiv190401180Y}. 
%This requires an NEP that is $20\times$ above the background-limited value. 

%. The MKID performance requirement is most clearly expressed and verified in a device under operational optical loading with NEP referring to input optical power at the lenslet. Additionally 

%Each of the EXCLAIM channels has a different optical loading, but the darkest channels receive the highest noise-inverse variance weight. 

% The number of isotropic $k$-modes in the volume is $N_k = V_{\rm survey} / (4 \pi^2) \cdot k^2 \Delta k$. 

 %The variance of the cross-power estimator is $\sigma^2[\hat P_\times (k)] = (2 N_k)^{-1} [P_\times^2 + P_{\rm IM} P_{\rm gal}]$ where $P_\times$ is the cross-power, $P_{\rm IM}$ is the intensity map auto-power, $P_{\rm gal}$ is the galaxy survey auto-power and $N_k$ is the number of survey $k$-modes in the bandpower. The detector noise enters the IM power spectrum $P_{\rm IM}$ as $\sigma_{\rm vox} V_{\rm vox}$ for voxels with volume $V_{\rm vox}$ and noise $\sigma_{\rm vox}$. To include the mode loss from beam and spectral response, define a transfer function \citep{2011ApJ...741...70L, 2014ApJ...786..111P, 2016ApJ...817..169L} in $k$ space (where {\it e.g.} beam convolution becomes multiplication), $T(k_\perp, k_\parallel) = e^{-(\sigma_\perp^2 k_\perp^2 - \sigma_\parallel^2 k_\parallel^2) / 2}$, where the factor of $2$ is due to the convolution on the intensity map but not the galaxy survey. Here $\sigma_\perp = \chi(z) \sigma_b$ for comoving radial distance $\chi(z)$ and Gaussian beam width $\sigma_b$, $\sigma_\parallel = [c/H(z)] \sigma_\nu (1+z)/\nu$ (where $H(z)$ is the Hubble constant and $c$ is the speed of light) for Gaussian spectral width $\sigma_\nu$ (which is a reasonable approximation to \mspec's passband). The transfer function of $P(k_\perp, k_\parallel)$ must then be weighted onto annuli of isotropic $|k|$ bins, which is equivalent to an effective number of modes $N^{\rm eff}_k = N_k \cdot \int_0^1 d\mu T^2(k, \mu)$, where $\mu = \cos(\theta)$ is the cos-angle of the ${\bf k}$ vector. Table~\ref{fig:sensitivity} shows results of this calculation for all EXCLAIM cross-powers. Variable noise from atmospheric lines is included as noise-inverse weighting by $w(\nu)$. 

%The majority of the sensitivity to the line amplitude comes from the highest spatial and spectral frequencies of the survey because these have the most signal variance and largest number of modes. In the spatial direction, this information is at acoustic frequencies of ${\sim}20$\,Hz, above the 1/f knee seen in \citet{2017A&A...601A..89B}. The lowest accessible $k$ mode will be limited by $1/f$ and residual correlated continuum emission. 

%\begin{thebibliography}{99}
%\bibitem{joynttaillefer02}
%R. Joynt and L. Taillefer, {\it Rev. Mod. Phys.} \textbf{74}, 235, (2002), DOI:10.1103/RevModPhys.74.235.
%\end{thebibliography}

